Variable decoupling and the Kolmogorov Superposition Theorem for rational functions

The goal of this paper is to show that for rational multivariate functions, the Kolmogorov Superposition Theorem (KST) involves several univariate functions, which can be written down by inspection. In other words, no computation is required for decoupling the variables of multivariate rational functions. The key tool for this development is the Loewner Framework for multivariate functions. Applications of this result involve the approximation of multivariate non-rational functions by low-complexity multivariate rational and polynomial functions.

==> ex1D/Delta_n.tex <==
\left[\begin{array}{ccc} 2 & 0 & 0\\[1mm] 0 & 3 & 0\\[1mm] 0 & 0 & 4 \end{array}\right]


==> ex1D/H.tex <==
\frac{\varS+1}{{\varS}^2+\varS+2}


==> ex1D/Vlambda.tex <==
\left[\begin{array}{ccc} 1 & 1 & 1\\[1mm] 1 & 2 & 3 \end{array}\right]


==> ex1D/c2.tex <==
\left[\begin{array}{c} 2\\[1mm] -8\\[1mm] 7 \end{array}\right]

